The kissing polynomials and their Hankel determinants

In this paper we investigate algebraic, differential and asymptotic properties of polynomials $p_n(x)$ that are orthogonal with respect to the complex oscillatory weight $w(x)=e^{i\omega x}$ on the interval $[-1,1]$, where $\omega>0$. We also investigate related quantities such as Hankel determinants and recurrence coefficients. We prove existence of the polynomials $p_{2n}(x)$ for all values of $\omega>0$, as well as degeneracy of $p_{2n+1}(x)$ at certain values of $\omega$ (called kissing points). We obtain detailed asymptotic information as $\omega\to\infty$, using recent theory of multivariate highly oscillatory integrals, and we complete the analysis with the study of complex zeros of Hankel determinants, using the large $\omega$ asymptotics obtained before.

==> refs_CDHI.tex <==
\begin{thebibliography}{99}
	
	
	\bibitem{asheim2014bounded}
	Asheim, A., Dea{\~n}o, A., Huybrechs, D., Wang, H.:
	A {G}aussian quadrature rule for oscillatory integrals on a bounded interval.
	{\it Discrete Contin. Dyn. Syst.} \textbf{34, 3}, 883--901 (2014).
	
	\bibitem{BCD2020}
	Barhoumi, A., Celsus, A. F., Dea\~{n}o, A.:
	Global phase portrait and large degree asymptotics for the kissing polynomials.
	{\it Stud. Appl. Math.} \textbf{147, 2} (2021), 448--526.
%	{\it https://arxiv.org/abs/2008.08724}.
	
	\bibitem{BCE_Jacobi}
	Basor, E., Chen, Y., Ehrhardt, T.:
	{P}ainlev\'{e} {V} and time-dependent {J}acobi polynomials
	{\it J. Phys. A: Math. Theor.} \textbf{43}, 015204 (25pp) (2010).
	
	\bibitem{brower93}
	Brower, R.C., Deo, N., Jain, S.C., Tan, C.I.:
	Symmetry breaking in the double-well Hermitian matrix model. 
	{\it Nucl. Pys.} \textbf{B405}, 166--187 (1993).
	
	\bibitem{Bleher08}
	Bleher, P. M.:
	Lectures on random matrix models. The Riemann--Hilbert approach.
	In {\it CRM Series in Mathematical Physics,}
	Springer, Berlin, 251--349 (2011).
	
	\bibitem{BleherItsdoublescaling}
	Bleher, P. M., Its, A.:
	Double scaling limit in the random matrix model: the Riemann-Hilbert approach.
	{\it Commun. Pure Appl. Math} \textbf{56}, 433--516 (2003).
	
	\bibitem{BleherIts}
	Bleher, P. M., Its, A.:
	Asymptotics of the partition function of a random matrix model.
	{\it Annales de l'Institut Fourier} \textbf{55, 6}, 1943--2000 (2005).
		
	\bibitem{BleherLiechty}
	Bleher, P., Liechty, K.:
	{\it Random Matrices and the Six-Vertex Model.}
	CRM Monograph Series, vol. 32.
	American Mathematical Society, 2013.
	
	\bibitem{brezinski1980formal}
	Brezinski, C.:
	{\it {P}ad{\'e}-type Approximation and General Orthogonal Polynomials.}
	Springer, Basel, 1980.
	
	\bibitem{calogerobook}
	Calogero, F.: 
	\textit{Classical many-body problems amenable to exact treatments: (solvable and/or integrable and/or linearizable) in One-, Two-, and Three~-Dimensional Space}. volume 66. Springer Science and Business Media, 2003. 
	
	\bibitem{celsus2020}
	Celsus, A.F., Silva, G.L.F.:
	Supercritical regime for the kissing polynomials. 
	\textit{J. Approx. Theory} \textbf{255} (2020), 105408.
	
	\bibitem{ChenIsmail}
	Chen, Y., Ismail, M. E. H.:
	Ladder operators and differential equations for orthogonal polynomials.
	\textit{J. Phys. A: Math. Gen.} \textbf{30}, 7817 (1997).

	\bibitem{chihara1978orthogonal}
	Chihara, T.:
	{\it An Introduction to Orthogonal Polynomials.}
	Gordon \& Breach, New York, 1978.

	\bibitem{LambertW}
	 Corless, R. M.,  Gonnet, G. H., Hare, D. E. G., Jeffrey, D. J., Knuth, D. E.:
	On the Lambert W function.
	 \textit{Adv. Comput. Math.} \textbf{5 (4)}, 329--359 (1996).
	 
	\bibitem{Dea2014asymp}
	Dea\~{n}o, A.:
	Large degree asymptotics of orthogonal polynomials with respect to an oscillatory weight on a bounded interval.
	{\it J. Approx. Theory} \textbf{186}, 33--63 (2014).
	
	\bibitem{DHquad}
	Dea\~{n}o, A. Huybrechs, D.:
	Complex Gaussian quadrature of oscillatory integrals.
	{\it Numer. Math.} \textbf{112 (2)}, 197--217 (2009).
	
	\bibitem{DHK}
	Dea\~{n}o, A., Huybrechs, D., Kuijlaars, A. B. J.:
	Asymptotic zero distribution of complex orthogonal polynomials associated with Gaussian quadrature.
	\textit{J. Approx. Theory} \textbf{162}, 2202--2224 (2010).
	
	\bibitem{DHI_book}
	Dea\~{n}o, A., Huybrechs, D., Iserles, A.:
	{\it Computing highly oscillatory integrals}
	SIAM, 2017.
	
	\bibitem{DKMVZ:1999}
	Deift, P., Kriecherbauer, T., McLaughlin, K. T.-R., Venakides, S., Zhou, X.:
	Strong Asymptotics of Orthogonal Polynomials with Respect to Exponential Weights.
	{\it Commun. Pure Appl, Math. LII, 1491--1552 (1999)}
	
	\bibitem{Deift2000OP}
	Deift, P.:
	{\it Orthogonal Polynomials and Random Matrices: A Riemann--Hilbert Approach.}
	Courant Lecture Notes in Mathematics, vol. 3.
	American Mathematical Society, 2000.
	
	\bibitem{DesrosiersLiu2014}
	Desrosiers, P., Liu, D.-Z.:
	Asymptotics for products of characteristic polynomials in classical $\beta$-ensembles.
	{\it Const. Approx.} \textbf{39}, 273--322 (2014).
	
	\bibitem{EdelmanStrang}
	Edelman, A., Strang, G.:
	Pascal matrices.
	{\it The American Mathematical Monthly} \textbf{111, 3}, 189--197 (2004)
	
	\bibitem{fokasdiscretepainleve}
	Fokas, A.S., Its, A.R., Kitaev, A.V.:
	Discrete Painlev\'e equations and their appearance in quantum gravity. \textit{Comm. Math. Physics.} \textbf{142, 2} 313 --344 (1991).
	
	\bibitem{fokasisomonodromy}
	Fokas, A.S., Its, A.R., Kitaev, A.V.:
	The isomonodromy approach to matrix models in 2D quantum gravity.	
	\textit{Comm. Math. Physics.} \textbf{147.2} 395 --430 (1992).
	
	\bibitem{gautschi2004opq}
	Gautschi, W.:
	{\it Orthogonal Polynomials: Computation and Approximation.}
	Clarendon Press, Oxford, 2004.
	
	\bibitem{GR1987}
	Gonchar, A. A. and Rakhmanov, E. A.:
	Equilibrium distributions and the rate of rational approximation of analytic functions.
	\textit{Mat. Sb. (N.S.)} \textbf{134, 3}, 306--352 (1987).
	
	\bibitem{HKL}
	Huybrechs, D., Kuijlaars, A. B. J., Lejon, N.:
	Zero distribution of complex orthogonal polynomials with respect to exponential weights.
	\textit{J. Approx. Theory} \textbf{184}, 28--54 (2014).
	
	\bibitem{ince_ODEs}
	Ince, E. L.:
	{\it Ordinary Differential Equations.}
	Dover Publications, New York, 1956.
	
	
	\bibitem{iserles2006multivariate}
	Iserles, A., N{\o}rsett, S. P.:
	Quadrature methods for multivariate highly oscillatory integrals using derivatives.
	{\it Math. Comp.} \textbf{255, 75}, 1233--1258 (2006).
	
	\bibitem{ismail2005orthogonal}
	Ismail, M. E. H.:
	{\it Classical and Quantum Orthogonal Polynomials in One Variable.}
	Cambridge University Press, Cambridge, 2005.

	\bibitem{ismailma}
	Ismail, M. E. H., Ma, W-X.:
	Equations of motion for zeros of orthogonal polynomials related to the Toda lattices.
	{\it Arab Journal of Mathematical Sciences \textbf{17, 1}, 1--10 (2011).}
	
	\bibitem{jimbomiwa2}
	Jimbo, M., Miwa, T.:
	Monodromy preserving deformation of linear ordinary differential equations with rational coefficients II.
	{\it Physica D} \textbf{2,3}, 407--448 (1981).
	
	\bibitem{KMcLVAV}
	Kuijlaars, A. B. J., McLaughlin, K. T.-R., Van Assche, W., Vanlessen, M.:
	The {R}iemann-{H}ilbert approach to strong asymptotics for
	orthogonal polynomials on {{$[-1,1]$}},
	\textit{Adv. Math.} \textbf{188, 2}, 337--398 (2004).
	
	\bibitem{KS}
	Kuijlaars, A. B. J., Silva, G. L. F.:
	$S$-curves in polynomial external fields. 
	\textit{J. Approx. Theory} \textbf{191}, 1--37 (2015).
	
	\bibitem{lejon16aao}
	Lejon, N. 
	{\it Analysis and applications of orthogonal polynomials with zeros in the complex plane.}
	PhD thesis, Department of Computer Science, KU Leuven, 2016.
	
	\bibitem{magnus1993}
	Magnus, A.P.:
	Asymptotics for the simplest generalized Jacobi polynomials recurrence coefficients from Freud's equations: numerical explorations. 
	\textit{Ann. Numer. Math.} \textbf{2, 1--4} pages 311-325 (1995).%. Special functions (Torino, 1993)
	
	\bibitem{magnus1995}
	Magnus, A.P.:
	Painlev\'e-type differential equations for the recurrence coefficients of semiclassical orthogonal polynomials. In \textit{Proceedings of the Fourth International Symposium on Orthogonal Polynomials and their Applications (Evian-Les-Bains, 1992)}, volume 57, pages 215-237, 1995. 
	
	\bibitem{MFR}
	Mart\'{\i}nez-Finkelshtein, A., Rakhmanov, E. A.:
	Do orthogonal polynomials dream of symmetric curves?
	\textit{Found. Comput. Math.} \textbf{16,6}, 1697--1736 (2016).
	
	\bibitem{NIST:DLMF}
	NIST Digital Library of Mathematical Functions
	http://dlmf.nist.gov/, Release 1.0.9 of 2014-08-29. 
	Online companion to \cite{Olver:2010:NHMF}.
	
	
	\bibitem{Olver:2010:NHMF}
	Olver, F. W. J., Lozier, D. W., Boisvert, R. F., Clark, C. W. (editors).:
	{\it NIST Handbook of Mathematical Functions.}
	Cambridge University Press, New York, NY, 2010. 
	Print companion to \cite{NIST:DLMF}.
	
	\bibitem{rainville1960special}
	Rainville, E. D.:
	{\it Special Functions.}
	Macmillan, New York, 1960.
	
	\bibitem{Rakhmanov}
	Rakhmanov, E. A.:
	Orthogonal polynomials and $S$-curves. In \textit{Recent Advances in Orthogonal Polynomials, Special Functions, and Their Applications}, Contemp. Math. \textbf{578},  195--239.
	%J. Arves\'u and G. L\'opez Lagomasino (eds.) Contemp. Math. \textbf{578},  195--239 (2012).%American Mathematical Society, Providence RI, 2011.
	
	\bibitem{Stahl}
	Stahl, H.
	Orthogonal polynomials with complex-valued weight function {I}, {II}.
	\textit{Constr. Approx.} \textbf{2, 3} 225--240, 241--251 (1986).
	
	\bibitem{Suetin}
	Suetin, S. P.:
	On the strong asymptotics of polynomials orthogonal with respect to a complex weight.
	\textit{Mat. Sb.}, \textbf{200, 1} 81--96 (2009).
	
	\bibitem{szego1939polynomials}
	Szeg\H{o}, G.: 
	{\it Orthogonal polynomials.}
	American Mathematical Society, Providence RI, 1939.
	
	\bibitem{van2017book}
	Van Assche, W.:
	\textit{Orthogonal Polynomials and Painlev\'e Equations}. Australian Mathematical Society Lecture Series, Volume 27. Cambridge University Press, 2018.
	
	\bibitem{wong2001asymptotic}
	Wong, R.:
	{\it Asymptotic Approximation of Integrals.}
	SIAM, Philadelphia, 2001.
\end{thebibliography}

